Refinement-based verification of sequential implementations of Stateflow charts

Simulink/Stateflow charts are widely used in industry for the specification of control systems, which are often safety-critical. This suggests a need for a formal treatment of such models. In previous work, we have proposed a technique for automatic generation of formal models of Stateflow blocks to support refinement-based reasoning. In this article, we present a refinement strategy that supports the verification of automatically generated sequential C implementations of Stateflow charts. In particular, we discuss how this strategy can be specialised to take advantage of architectural features in order to allow a higher level of automation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{65}
\providecommand{\publicationstatus}{J. Derrick , E.A. Boiten, S. Reeves (Eds.):\\
Refinement Workshop 2011.
\\
EPTCS 55, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.55.5}{10.4204/EPTCS.55.5}}
\pdfoutput=1

